Target Domain Data induces Negative Transfer in Mixed Domain Training with Disjoint Classes

In practical scenarios, it is often the case that the available training data within the target domain only exist for a limited number of classes, with the remaining classes only available within surrogate domains. We show that including the target domain in training when there exist disjoint classes between the target and surrogate domains creates significant negative transfer, and causes performance to significantly decrease compared to training without the target domain at all. We hypothesize that this negative transfer is due to an intermediate shortcut that only occurs when multiple source domains are present, and provide experimental evidence that this may be the case. We show that this phenomena occurs on over 25 distinct domain shifts, both synthetic and real, and in many cases deteriorates the performance to well worse than random, even when using state-of-the-art domain adaptation methods.

==> notes.tex <==
\begin{document}
experiments already done: 
\begin{itemize}
    \item VLCS
    \item PACS
    \begin{itemize}
        \item resnet
        \item convnext
        \item vit-b
    \end{itemize}
    \item ColoredMNIST variant - show the in-classes + out-classes. 
    \item VisDA 2017 
\end{itemize}

some potential experiments
\begin{itemize}
    \item domainNet? cancelled. 
    \item domain shift methods? we can try to use domainbed or something... deprioritized past mixup. 
    \item proportionality experiment
    \item obj det - cancelled. 
    \item mixup \citet{zhang2017mixup}, augmentations. 
    \item randomize labels in the target training classes, see if you have no transfer. This only kinda matters, jsut shows that decision tree effect happens. 
    \item random noise for the images instead - funny, but probably not needed.  
    \item PC -> A. this means that \textbf{target domain data} induces this. 
\end{itemize}



\section{general outline (delete me later)}

[intro, related-work, notation 2.5-3 pages]

1) it's very common for scenarios where multiple source datasets are combined to create a dataset for training.

2) oftentimes, this arises by having only limited data from the target domain for some classes, and augmenting rare or no class counts with another surrogate dataset that is hopefully similar to the target. 

3) However, we find that adding target domain data to the surrogate classes induces significant negative transfer, here's a colored mnist experiment walking through this. 

ColoredMNIST [2 pages, conf matrix, experimental setup]

4) T[0-4], S[5-9], let's imagine first of all that the labels of T are completely random. in this case, we expect T[5-9] to be about as good as S[5-9] -> T. However, we actually do much worse. In fact, the model is randomly putting things in the T bucket. This kinda makes sense, since we had no information about T.  [this invites questions about unsupervised usage of T[0-4].] We might have to do some experiment with uda where T[0-4] is the data. 

5) Ok, what if you give class information to this? T[0-4], S[5-9] with classes - oh wow it does the poorly, the same as random labels - it's still randomly putting things in the T bucket. Using target data does not help, regardless of supervision. Does this invite using supervised domain adaptation methods?

6) However, if you use S2[0-4], S[5-9], this actually does quite well. The presence of classes 0-4 do not harm performance; it is the fact that those labels are from / close to domain T that damages performance.

[Generalization to other datasets. PACS, VLCS, etc. 1-1.5 page]

7) Look, this happens on not just MNIST datasets, which have very sparse features, but also on more complicated datasets, and on more complicated models. Here are 25 domain shifts. (PACS, VLCS, VisDA), and 3 models (convnext, resnet18, ViT). This is not just something that happens on CNN's, it is a general problem in domain adaptation.

[Mix-Up, and experiments 1-2 page]

8) Well what can you do? One potential solution is mixup. Here's some attempts at overcoming this. Use mixup, whenever you do something like this.

[Conclusion] 0.5 pages. 

\begin{enumerate}
    \item proportion experiment
    \item confusion matrix generation
    \item umap generation
    \item paper writing
    \begin{enumerate}
        \item intro
        \item related work
        \item background/problem setting
        \item colored mnist
        \item experiment setup
        \item results and discussion
        \item solution. 
        \item conclusion
    \end{enumerate}
    \item table generation
    \item stacked bar chart generation
    
\end{enumerate}

\end{document}
